Neural Face Skinning for Mesh-agnostic Facial Expression Cloning

Accurately retargeting facial expressions to a face mesh while enabling manipulation is a key challenge in facial animation retargeting. Recent deep-learning methods address this by encoding facial expressions into a global latent code, but they often fail to capture fine-grained details in local regions. While some methods improve local accuracy by transferring deformations locally, this often complicates overall control of the facial expression. To address this, we propose a method that combines the strengths of both global and local deformation models. Our approach enables intuitive control and detailed expression cloning across diverse face meshes, regardless of their underlying structures. The core idea is to localize the influence of the global latent code on the target mesh. Our model learns to predict skinning weights for each vertex of the target face mesh through indirect supervision from predefined segmentation labels. These predicted weights localize the global latent code, enabling precise and region-specific deformations even for meshes with unseen shapes. We supervise the latent code using Facial Action Coding System (FACS)-based blendshapes to ensure interpretability and allow straightforward editing of the generated animation. Through extensive experiments, we demonstrate improved performance over state-of-the-art methods in terms of expression fidelity, deformation transfer accuracy, and adaptability across diverse mesh structures.

==> fig_tex/01_intro.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/01_intro.pdf}
\end{center}
\vspace{-1mm}
\caption[Illustration of the key idea]{
    \textbf{Illustration of the key idea.} The global expression code (c) represents the deformation from neutral face (a) to expressed face (b), where the color indicates the activation. Previous methods use global expression code (c) uniformly across all vertices (d), whereas our method uses localized expression code (d).
}
\vspace{-5mm}
\label{fig:intro}
\end{figure}




==> fig_tex/02_goal.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/02_goal.png}
\end{center}
\vspace{-1mm}
\caption[Comparison of comparative methods]{
    \textbf{Visual comparison of the methods.} 
    Our method enables mesh-agnostic audio-driven facial animation by leveraging the advantages of an audio-driven method and the recent deformation transfer method.
     % The proposed method (b) can animate any 3D face mesh given an audio input, without being constrained to a certain topology, while previous methods~\cite{xing2023codetalker,fan2022faceformer,stan2023facediffuser} (a) are bounded by the trained mesh topology.
     \todo{change table to : coeff-based, vertex-based, Ours}
}
\vspace{-6mm}
\label{fig:compare_goal}
\end{figure}




==> fig_tex/03_segment_prediction.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=0.9\linewidth]{fig/04_segment.pdf}
\end{center}
\caption[Visualization of face skinning weight on the ICT face mesh and various unseen meshes]{
Visualization of face skinning weight on the ICT face mesh and various unseen meshes. We extracted the maximum value in $z_{Skin}$ for each vertex and calculated the mode value on each triangle for the rendering. \small{© Face model: ICT~\cite{li2020ictface}, BIWI~\cite{fanelli2013biwi}, VOCA2019, Multiface~\cite{wuu2022multiface}, meryproject.com, 2023 AnimSchool}
% The upper row indicates the result from ICT, and the lower row indicates the result from VOCA~\cite{VOCA2019} and Multiface~\cite{wuu2022multiface}.
% \todo{will be moved to supplementary}
}
\label{fig:face_segment}
\end{figure}

% \clearpage

==> fig_tex/05_control.tex <==
\begin{figure}[t]
\begin{center}
\includegraphics[width=.9\linewidth]{fig/05_control.pdf}
\end{center}
\caption[Results of expression control on arbitrary face mesh]{
    Results of expression control on arbitrary face mesh. Our method can animate various face meshes based on the ICT blendshape coefficient. The similarity of the facial movement can be observed.
}
\vspace{-3mm}
\label{fig:control}
\end{figure}


==> fig_tex/05_ict_segment.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.6\linewidth]{fig/04_ICT_segment-all.png}
% \includegraphics[width=\linewidth]{fig/04_ICT_segment.png}
\end{center}
\caption[Manually defined face segments on ICT-Facekit]{
Manually defined $20$ face segments on the ICT-Facekit~\cite{li2020ictface} model. Visualization of the per-vertex label (top) and the face segment mapped on UV of the ICT model (bottom).
}
\label{fig:ict_segment}
\end{figure}


==> fig_tex/05_implicit_segment.tex <==
\begin{figure}[h]
\begin{center}
\includegraphics[width=0.8\linewidth]{fig/05_implicit_segment.png}
\end{center}
\caption[Visualization of Implicitly learned segment]{
Visualization of the implicitly learned segments on various meshes, with examples from ICT, Multiface, and BIWI datasets, arranged from top to bottom.
}
\label{fig:implicit_seg}
\end{figure}


==> fig_tex/07_alignment.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_rescaling.pdf}
\end{center}
\vspace{-2mm}
\caption[Visualization of face mesh alignment]{
    Visualization of face mesh alignment. From the left, the meshes are from ICT, VOCASET, and BIWI.
}
\vspace{-4mm}
\label{fig:alignment}
\end{figure}

==> fig_tex/07_editing.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_editing.pdf}
\end{center}
\caption[Results of expression editing]{
    Results of expression editing. The facial animation was generated using the ICT blendshape coefficient and edited by modifying the coefficient. The corresponding blendshape used for the editing is written on the left with quotation marks. The color indicates the MSE computed against the initially generated animation.
}
\label{fig:editing}
\end{figure}


==> fig_tex/07_editing_stack.tex <==

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_editing_stack.pdf}
\end{center}
\caption[Results of expression editing]{
    Results of expression editing 2. The expression can be added while maintaining the local expression.
}
\label{fig:editing_stack}
\end{figure}


==> fig_tex/07_expression_deform.tex <==

\begin{figure*}[th]
\begin{center}
\includegraphics[width=.9\linewidth]{fig/07_expression_53_deform.pdf}
\end{center}
\caption[Deformation based on global expression code]{
    Visualization of the deformation based on the first 53 dimensions of global expression code, which are interpretable.
}
\label{fig:exp_deform}
\end{figure*}


==> fig_tex/07_user_study.tex <==

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_user_study_survey.pdf}
\end{center}
\caption[User study questionnaire]{
    A sample of the questionnaire from the user study.
}
\label{fig:user_study_survey}
\end{figure}


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_user_study_similarity.pdf}
\end{center}
\caption[The result of User study for expression similarity]{
    The result of user study for expression similarity.
}
\label{fig:user_similarity}
\end{figure}


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{fig/07_user_preference.pdf}
\end{center}
\caption[The result of user study for the overall preference]{
    The result of user study for the overall preference.
}
\label{fig:user_preference}
\end{figure}


==> table_tex/02_goal.tex <==

\begin{table}[t]
\captionof{table}[Visual comparison of the methods.]{
   \textbf{Visual comparison of the methods.} 
   Our method generates realistic speech-driven facial animation and allows easy editing of the generated animation for any arbitrary face mesh.
}
\vspace{-1mm}
\centering
\resizebox{\linewidth}{!}{

\begin{tabular}{l|ccc}
\toprule
        & \begin{tabular}[c]{@{}c@{}}Vertex-based\\ method\end{tabular} 
        & \begin{tabular}[c]{@{}c@{}}Coefficient-based\\ method\end{tabular} 
        & \begin{tabular}[c]{@{}c@{}} Ours \end{tabular} \\ 
\midrule
% \midrule
\begin{tabular}[c]{@{}l@{}}Natural and realistic\\ lip-sync animation\end{tabular} 
    & \LARGE \textcolor{green}{\ding{51}} 
    & \LARGE\textcolor{red}{\ding{55}} 
    & \LARGE\textcolor{green}{\ding{51}}     \\
\midrule
\begin{tabular}[c]{@{}l@{}}Easy editing and\\ detailed control\end{tabular} 
    & \LARGE\textcolor{red}{\ding{55}} 
    & \LARGE\textcolor{green}{\ding{51}} 
    & \LARGE\textcolor{green}{\ding{51}}     \\
\midrule
\begin{tabular}[c]{@{}l@{}}Compatible with mesh in\\ various shapes and structures\end{tabular} 
    & \LARGE\textcolor{red}{\ding{55}} 
    & \LARGE\textcolor{red}{\ding{55}} 
    & \LARGE\textcolor{green}{\ding{51}}     \\
\bottomrule
\end{tabular}

\label{tab:compare_goal}
}
\end{table}

==> table_tex/04_face_segment.tex <==

\begin{table}[h]
\vspace{-1mm}
\captionof{table}[Face segmentation]{
    Face segment prediction accuracy on the ICT test dataset.
}
\vspace{-1mm}
\centering
\begin{tabular}{lc}
    \toprule 
    Method      & Precision  \\
    \midrule
    Ours        & 99.97\%  \\
    \bottomrule
\end{tabular} 
\vspace{-3mm}
% \vspace{-6mm}
\label{tab:face_seg}
\end{table}


==> table_tex/04_lip_vertex.tex <==

% \begin{table}[h]
% \captionof{table}[Facial expression retargeting]{
%     Facial expression retargeting results on various face meshes.
% }
% \centering
% \begin{tabular}{lcccc}
% \toprule 
% \multirow{2}{*}{Method} & \multicolumn{4}{c}{LVE $\downarrow (\times 10^{-3})$ }   \\ \cline{2-5}
%                         & ICT   & Multiface & VOCA  & BIWI \\ \cline{1-5}
% NFR (pretrained)        & 7.496 &  9.329    & 5.259 & 17.16\\
% NFR*                    & 7.493 & 10.965    & 5.665 & 4.769 \\
% Ours (w/o seg)          & 2.114 & 10.927    & 4.223 &  \\
% Ours                    & 3.881 &  7.759    & 3.879E-03 & 5.008E-03 \\
% \bottomrule
% \end{tabular}\label{tab:lip_vertex}
% \end{table}


\begin{table}[h]
\captionof{table}[Lip vertex error]{
    Comparison with state-of-the-art methods using benchmark datasets. The method that is constrained to VOCASET~\cite{VOCA2019}, BIWI~\cite{fanelli2013biwi} and ICT~\cite{li2020ictface} is denoted with superscripts `${V}$',`${B}$' and `${I}$', respectively.
}
\centering
\begin{tabular}{lccc}
\toprule 
\multirow{2}{*}{Method} & \multicolumn{3}{c}{LVE $\downarrow (\times 10^{-3}mm)$ }\\ \cline{2-4}
                        & VOCASET          & BIWI            & ICT             \\  \cline{1-4}
$\text{FaceFormer}^{V}$ & 4.9503           &    -            &  -              \\
$\text{CodeTalker}^{V}$ & \textbf{4.8836}  &    -            &  -              \\  \midrule
$\text{FaceFormer}^{B}$ &   -              & 4.1710          &  -              \\
$\text{CodeTalker}^{B}$ &   -              & \textbf{4.1203} &  -              \\  \midrule
$\text{FaceFormer}^{I}$ &   -              & -               & 0.9473          \\
$\text{CodeTalker}^{I}$ &   -              & -               & 1.8430          \\  \midrule
Ours                    & 5.4869  & 5.7374          & \textbf{0.7006} \\
\bottomrule
\end{tabular}\label{tab:lip_vertex}
\vspace{-1mm}
\end{table}
